A bound preserving cut discontinuous Galerkin method for one dimensional hyperbolic conservation laws

In this paper we present a family of high order cut finite element methods with bound preserving properties for hyperbolic conservation laws in one space dimension. The methods are based on the discontinuous Galerkin framework and use a regular background mesh, where interior boundaries are allowed to cut through the mesh arbitrarily. Our methods include ghost penalty stabilization to handle small cut elements and a new reconstruction of the approximation on macro-elements, which are local patches consisting of cut and un-cut neighboring elements that are connected by stabilization. We show that the reconstructed solution retains conservation and order of convergence. Our lowest-order scheme results in a piecewise constant solution that satisfies a maximum principle for scalar hyperbolic conservation laws. When the lowest order scheme is applied to the Euler equations, the scheme is positivity preserving in the sense that positivity of pressure and density are retained. For the high-order schemes, suitable bound preserving limiters are applied to the reconstructed solution on macro-elements. In the scalar case, a maximum principle limiter is applied, which ensures that the limited approximation satisfies the maximum principle. Correspondingly, we use a positivity preserving limiter for the Euler equations and show that our scheme is positivity preserving. In the presence of shocks, additional limiting is needed to avoid oscillations, hence we apply a standard TVB limiter to the reconstructed solution. The time step restrictions are of the same order as for the corresponding discontinuous Galerkin methods on the background mesh. Numerical computations illustrate accuracy, bound preservation, and shock capturing capabilities of the proposed schemes.

==> cutcellatBC.tex <==
\section{Numerical results on the mesh non-aligned boundaries}
\fp{In this Appendix, we give two examples for the case of  non-aligned boundaries. The physical domain $[x_l,x_r]$ is immersed in the background mesh. We take the computational domain as  $[x_L,x_R]$ with $x_L=x_l-(1-\alpha)h,x_R=x_r+(1-\alpha h)$, which is discritized by the uniform grid $x_L=x_0<x_1<\cdots<x_N<x_{N+1/2}=x_R$. Thus, same as in \cite{YangInverseLB}, two unfitted cells with size $\alpha h$ are listed on the boundary.   
}
\fp{
The first case is the linear advection $u_t+u_x=0$ with inflow boundary condition $g(t)$ on the left boundary $x=0$ and outflow boundary condition on the right boundary $x=1$ as in \cite{YangInverseLB}.  The initial condition is $u(x,0)=0$ and 
\begin{align}
g(t)= \begin{cases}1, & t \leq 0.5, \\ 0, & t>0.5.\end{cases}
\end{align}
Same as  in \cite{YangInverseLB},  we take $\alpha=0.01$ and solve the problem up to $t=0.75$, when the solution has two discontinuities located at $x=0.25,x=0.75$ respectively.  In Figure \ref{fig:linear:nonsmoothbc}, the results show that our proposed scheme on the mesh not aligned with boundary preserves maximum principle and does not introduce additional numerical oscillations,  when handling strong discontinuities near cut cells.
\begin{figure}[!htp]
\centering
\includegraphics[width=2.0in]{Linear_NonsmoothBC_CutOut_P1_Macro1_Bound1_Alpha001_CLFNGLmo.eps}
\includegraphics[width=2.0in]{Linear_NonsmoothBC_CutOut_P2_Macro1_Bound1_Alpha001_CLFNGLmo.eps}
\includegraphics[width=2.0in]{Linear_NonsmoothBC_CutOut_P3_Macro1_Bound1_Alpha001_CLFNGLmo.eps}
\caption{Example 5.1: numerical solutions on the mesh not aligned with boundary  for linear equation \eqref{eq:test:linear} with non-smooth boundary condition at t = 0.75. $P^1,P^2,P^3$ approximation from left to right. }\label{fig:linear:nonsmoothbc}
\end{figure}
}


\fp{
In the second case, the two blast wave \cite{woodward1984numerical} with shocks  is  simulated by our proposed scheme for Euler equations.  We solve the problem on the mesh non-aligned boundaries, same as in \cite{TAN20108144}. 
The initial data are
\begin{align}
\boldsymbol{u}(x, 0)= \begin{cases}
\boldsymbol{u}_L & 0<x<0.1, \\ 
\boldsymbol{u}_M & 0.1<x<0.9, \\
 \boldsymbol{u}_R & 0.9<x<1,
 \end{cases}
\end{align}
where $\rho_L=\rho_M=\rho_R=1, u_L=u_M=u_R=0, p_L=10^3, p_M=10^{-2}, p_R=10^2$.  The solid wall boundary conditions are used at both $x=0$ and $x=1$. 
Multiple reflections of shocks and rarefactions are involved  off the walls in the solution of this problem. In addition, there are a variety of interactions between shock waves and rarefaction waves, as well as between these waves and contact discontinuities.  We solve this problem by our proposed positivity-preserving scheme up to $t=0.038$. The numerical solution of density is shown in Figure \ref{fig:euler:twoblastwave}.  We use the solution from the standard DG method on the uniform mesh  with $h = 1/6400$,  where the reflection boundary condition is used  at both boundaries.  We can see that our proposed scheme can capture the structure of the solution well and preserve the positivity of density and pressure in our simulation. 
\begin{figure}[!htp]
\centering
\includegraphics[width=2.0in]{Euler_twoblastwave_CutDG_P1_alpha001_macro1_bound1.eps}
\includegraphics[width=2.0in]{Euler_twoblastwave_CutDG_P2_alpha001_macro1_bound1.eps}
\includegraphics[width=2.0in]{Euler_twoblastwave_CutDG_P3_alpha001_macro1_bound1.eps}
\caption{Example 5.3: numerical approximations of density at $t=0.038$ for two blast wave problem. Circle: numerical solution from our proposed scheme. Solid: reference solution from the standard DG method.  $P^1,P^2,P^3$ approximation from left to right. }\label{fig:euler:twoblastwave}
\end{figure}
}
